Top of the Batch: Interviews and the Match

Most doctors in the NRMP are matched to one of their most-preferred internship programs. Since various surveys indicate similarities across doctors' preferences, this suggests a puzzle. How can nearly everyone get a position in a highly-desirable program when positions in each program are scarce? We provide one possible explanation for this puzzle. We show that the patterns observed in the NRMP data may be an artifact of the interview process that precedes the match. Our analysis highlights the importance of interactions occurring outside of a matching clearinghouse for resulting outcomes, and casts doubts on analysis of clearinghouses that take reported preferences at face value.

==> tbl/AltTable.tex <==
\begin{tabular}{lccccccc}
    \toprule
    \multicolumn{3}{l}{\textbf{NRMP Data}}  &  \multicolumn{3}{c}{Conditional on Match} & Unmatched\\ \cmidrule{4-6}
    
    & & & Exp. Rank & Top & Top-4 \\ \midrule
     2010--20& & & $3.1^\dagger$& 0.51  & 0.84  &  0.23 \\
     & &  &  \footnotesize{(0.2)} & \footnotesize{(0.02)} & {\footnotesize{(0.01)}} & \footnotesize{(0.03)} \\
     \midrule
     \multicolumn{3}{l}{\textbf{Simulations:}}\\
     \midrule
$\lambda=\nicefrac{1}{5}$   & $N=50$    & TA-GS &  2.0      & 0.47  & 0.95  & 0.05  \\
                            &           & SI-GS &  2.0      & 0.47  & 0.96  & 0.06  \\
                            &           & Tr-GS &  2.2      & 0.38  & 0.97  & 0.12  \\
                            &           & GS    &  5.5      & 0.19  & 0.57  & 0.00  \\ \cmidrule{2-7}
                            & $N=1700$  & TA-GS &  2.1      & 0.48  & 0.95  & 0.05  \\
                            &           & SI-GS &  2.0      & 0.46  & 0.96  & 0.06  \\
                            &           & Tr-GS &  2.3      & 0.35  & 0.92  & 0.38  \\
                            &           & GS    & 24.1      & 0.05  & 0.17  & 0.00  \\ \midrule
$\lambda=\nicefrac{4}{5}$   & $N=50$    & TA-GS &  2.2      & 0.35  & 0.95  & 0.04  \\
                            &           & SI-GS &  2.2      & 0.38  & 0.95  & 0.04  \\
                            &           & Tr-GS &  3.4      & 0.14  & 0.97  & 0.76  \\
                            &           & GS    &  22.0     & 0.03  & 0.12  & 0.00  \\\cmidrule{2-7}
                            & $N=1700$  & TA-GS &  2.1      & 0.43  & 0.95  & 0.05  \\
                            &           & SI-GS &  2.1      & 0.43  & 0.95  & 0.06  \\
                            &           & Tr-GS &  3.9      & 0.05  & 0.58  & 0.97  \\
                            &           & GS    &  645.4    & 0.00  & 0.01  & 0.00  \\
    \bottomrule
    \end{tabular}

==> tbl/Table2.tex <==
\begin{tabular}{lcccc c}\toprule
Outcome & \multicolumn{4}{c}

Source & $\la^D=\la^H$ & Exp. Rank & Top & Top-4 &   Unmatched \\ \midrule
 \textbf{NRMP:}\\ 
 2019 & & $3.3^\dagger$ & 0.49  & 0.85    &  0.19 \\ 2018 & & $3.2^\dagger$ & 0.50   & 0.85  &  0.20 \\
 \midrule
\textbf{SIGS}\\
 & 0.2 &  2.0 (13.3) & 0.46 (0.26) & 0.95 (0.62) & 0.06 \\
 & 0.4 & 2.0 (59.0)  & 0.47 (0.09) & 0.95 (0.26)  & 0.06 \\
 & 0.6 & 2.0 (239.4)  & 0.45 (0.01) & 0.95 (0.05)  & 0.06 \\
 & 0.8 &  2.0 (579.9) & 0.45 (0.00)  & 0.95 (0.01) & 0.05 \\ \midrule
\textbf{Truncated:}\\ 
 & 0.2 & 2.4  & 0.34  & 0.90   & 0.18 \\
 &0.4  & 2.9  & 0.21  & 0.82   & 0.50 \\
 & 0.6 & 3.3  & 0.12  & 0.74   & 0.83 \\
 & 0.8 & 4.0  & 0.05 &  0.57   & 0.97 \\ \bottomrule
\end{tabular}

==> tbl/Table2_1700_10.tex <==
\begin{tabular}{lccccc}\toprule
Source & $\la^D=\la^H$ & Exp. Rank & Top & Top-4 &   Unmatched \\ \midrule
 \textbf{NRMP:}\\ 
 2020 & & $3.4^\dagger$ & 0.48  & 0.84  &  0.18 \\ 
 2019 & & $3.3^\dagger$ & 0.49  & 0.85    &  0.19 \\ 2018 & & $3.2^\dagger$ & 0.50   & 0.85  &  0.20 \\
 \midrule
\textbf{SIGS}\\
 & 0.2 &  2.0 (13.3) & 0.46 (0.26) & 0.95 (0.62) & 0.06 \\
 & 0.4 & 2.0 (59.0)  & 0.47 (0.09) & 0.95 (0.26)  & 0.06 \\
 & 0.6 & 2.0 (239.4)  & 0.45 (0.01) & 0.95 (0.05)  & 0.06 \\
 & 0.8 &  2.0 (579.9) & 0.45 (0.00)  & 0.95 (0.01) & 0.05 \\ \midrule
\textbf{Truncated:}\\ 
 & 0.2 & 2.4  & 0.34  & 0.90   & 0.18 \\
 &0.4  & 2.9  & 0.21  & 0.82   & 0.50 \\
 & 0.6 & 3.3  & 0.12  & 0.74   & 0.83 \\
 & 0.8 & 4.0  & 0.05 &  0.57   & 0.97 \\ \bottomrule
\end{tabular}

==> tbl/Table2_50.tex <==
\begin{tabular}{lccccc}\toprule
Source & $\la^D=\la^H$ & Exp. Rank & Top & Top-4 &   Unmatched \\ \midrule
\textbf{SIGS}\\
& 0.0 &  2.9 (4.1) & 0.34 (0.28) & 0.81 (0.72)  & 0.02 \\ 
 & 0.2 &  2.8 (5.0) & 0.34 (0.27) & 0.82 (0.67) & 0.02 \\
 & 0.4 & 2.9 (8.7) & 0.32 (0.17) & 0.81 (0.49)  & 0.02 \\
& 0.6 & 3.1 (15.1)& 0.28 (0.07) & 0.78 (0.25)   & 0.02 \\
& 0.8 &  3.6 (21.6) & 0.19 (0.03)  & 0.69 (0.13)  & 0.01 \\ \midrule
\textbf{Truncated:}\\ 
 & 0.0 & 3.1  & 0.31  & 0.78   & 0.03 \\ 
 & 0.2 & 3.3  & 0.27  & 0.74   & 0.05 \\
 & 0.4 & 4.2  & 0.18  & 0.60  & 0.15 \\
 & 0.6 & 5.4  & 0.10  & 0.41  & 0.37 \\
 & 0.8 & 6.2  & 0.08  &  0.32  & 0.62 \\ \bottomrule
\end{tabular}

==> tbl/Table2_old.tex <==
\begin{tabular}{l|cccc|c}\toprule
Rank difference & First & Second & Third & Fourth & Unmatched \\ \midrule
$\la^D=\la^H=$ 0.2 & 12.3 & 7.4  & 3.9  & 2.2 & 2.5 \\
$\la^D=\la^H=$ 0.3 & 18.6 & 11.6 & 6.5  & 3.7 & 2.5 \\
$\la^D=\la^H=$ 0.4 & 24.7 & 15.6 & 10.2 & 6.2 & 2.7 \\
$\la^D=\la^H=$ 0.5 & 28.5 & 19.1 & 12.2 & 7.3 & 2.7 \\
$\la^D=\la^H=$ 0.6 & 29.6 & 20.5 & 13.9 & 9.1 & 2.6 \\ \bottomrule
\end{tabular}

